Pathologies of Neural Models Make Interpretations Difficult

One way to interpret neural model predictions is to highlight the most important input features---for example, a heatmap visualization over the words in an input sentence. In existing interpretation methods for NLP, a word's importance is determined by either input perturbation---measuring the decrease in model confidence when that word is removed---or by the gradient with respect to that word. To understand the limitations of these methods, we use input reduction, which iteratively removes the least important word from the input. This exposes pathological behaviors of neural models: the remaining words appear nonsensical to humans and are not the ones determined as important by interpretation methods. As we confirm with human experiments, the reduced examples lack information to support the prediction of any label, but models still make the same predictions with high confidence. To explain these counterintuitive results, we draw connections to adversarial examples and confidence calibration: pathological behaviors reveal difficulties in interpreting neural models trained with maximum likelihood. To mitigate their deficiencies, we fine-tune the models by encouraging high entropy outputs on reduced examples. Fine-tuned models become more interpretable under input reduction without accuracy loss on regular examples.

==> sections/60-related.tex <==
\section{Related Work}
\label{sec:related}

\fscomment{this section is merged into 50-discussion, keeping the file for the
comments}

We now review relevant previous work in interpretability methods, their
shortcomings, and mitigation techniques.

\jbgcomment{Expand now that we have more room. }

\ewcomment{Adversarial perturbations can also be enhanced by feature attribution
methods~\cite{mudrakarta2018understand} }
\ewcomment{We showed that the input reduction process found words that did not
align with human perception. ~\cite{Khashabi2017learning} trained a model to
classify what words a human would deem are important. This improved the
performance of a downstream model. }

Finally, the reduced examples highlight a model limitation that may be
exploited by an adversary.  Other ways to expose these types of
examples in \nlp{} have taken the form of word and character-level
modifications~\cite{papernot2016crafting, ebrahimi2017hotflip,
belinkov2017synthetic}. Additionally, neural models for reading
comprehension appear to be overly stable to non-destructive additive
changes such as inserting distractors~\cite{jia2017adversarial}. Our
work has shown models can remain highly confident even when crucial
information is \emph{removed} from their input.

\ewcomment{maybe add sear?}

